Don't Go To Extremes: Revealing the Excessive Sensitivity and Calibration Limitations of LLMs in Implicit Hate Speech Detection

The fairness and trustworthiness of Large Language Models (LLMs) are receiving increasing attention. Implicit hate speech, which employs indirect language to convey hateful intentions, occupies a significant portion of practice. However, the extent to which LLMs effectively address this issue remains insufficiently examined. This paper delves into the capability of LLMs to detect implicit hate speech (Classification Task) and express confidence in their responses (Calibration Task). Our evaluation meticulously considers various prompt patterns and mainstream uncertainty estimation methods. Our findings highlight that LLMs exhibit two extremes: (1) LLMs display excessive sensitivity towards groups or topics that may cause fairness issues, resulting in misclassifying benign statements as hate speech. (2) LLMs' confidence scores for each method excessively concentrate on a fixed range, remaining unchanged regardless of the dataset's complexity. Consequently, the calibration performance is heavily reliant on primary classification accuracy. These discoveries unveil new limitations of LLMs, underscoring the need for caution when optimizing models to ensure they do not veer towards extremes. This serves as a reminder to carefully consider sensitivity and confidence in the pursuit of model fairness.

==> _fig/conf_compare_consistency_logit.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=6.66in]{_fig/experiment/compare-consistency-logit.pdf}
    % \vspace{-20mm}
    \caption{compare conf consistency vs logit, on gpt35, sbic}
    \label{fig: conf-compare-consistency-logit}
\end{figure*}

==> _fig/conf_compare_verbal_logit.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=6.66in]{_fig/experiment/compare-verbal-logit.pdf}
    % \vspace{-20mm}
    \caption{compare conf verbal vs logit, on llama, implicit}
    \label{fig: conf-compare-verbal-logit}
\end{figure*}

==> _fig/conf_over_calibrate.tex <==
\begin{figure}
    \centering
    \includegraphics{_fig/experiment/over-calibrate.pdf}
    \vspace{-20mm}
    \caption{conf-over-calibrate}
    \label{fig: conf-over-calibrate}
\end{figure}

==> _fig/ece_llama_implicit_3method.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=6.66in]{_fig/experiment/ece_llama_implicit_3method.pdf}
    % \vspace{-20mm}
    \caption{prob distribution and ece llama implicit 3 method}
    \label{fig: ece-llama-implicit-3method}
\end{figure*}

==> _fig/ece_llama_toxigen_3method.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=6.66in]{_fig/experiment/ece_llama_toxigen_3method.pdf}
    % \vspace{-20mm}
    \caption{prob distribution and ece llama toxigen 3 method}
    \label{fig: ece-llama-toxigen-3method}
\end{figure*}

==> _fig/ece_mixtral_implicit_3method.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=6.66in]{_fig/experiment/ece_mixtral_implicit_3method.pdf}
    % \vspace{-20mm}
    \caption{prob distribution and ece mixtral implicit 3 method}
    \label{fig: ece-mixtral-implicit-3method}
\end{figure*}

==> _tables/conf_combine.tex <==
\begin{table*}[]
% \scalebox{0.8}
%     {
\setlength{\tabcolsep}{1mm}{
    \begin{tabular}{c}
    \begin{tabular}
    {
        S
        % P{min=0.6518, max=0.686, first color=green, second color=orange}{}
        P{min=0.5648, max=0.6374, first color=green, second color=orange}{}
        P{min=0.0812, max=0.1735, first color=orange, second color=green}{}
        P{min=0.2325, max=0.2763, first color=orange, second color=green}{}
        % P{min=0.7844, max=0.7949, first color=green, second color=orange}{}
        P{min=0.5861, max=0.7486, first color=green, second color=orange}{}
        P{min=0.0569, max=0.1029, first color=orange, second color=green}{}
        P{min=0.1652, max=0.1811, first color=orange, second color=green}{}
        % P{min=0.9176, max=0.9322, first color=green, second color=orange}{}
        P{min=0.7268, max=0.8886, first color=green, second color=orange}{}
        P{min=0.0288, max=0.1808, first color=orange, second color=green}{}
        P{min=0.0471, max=0.0891, first color=orange, second color=green}{}}
        & \multicolumn{3}{c}{implicit}  & \multicolumn{3}{c}{sbic}  & \multicolumn{3}{c}{toxigen}           \\
    \multicolumn{1}{c}{conf}         & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}          & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}      \\
    \multicolumn{10}{c}{LLaMA-2-7b}            \\
    {verbal}  & 0.5648 & 0.0812 & 0.2325  & 0.5861 & 0.0569 & 0.1811  & 0.7685 & 0.1808 & 0.0891 \\
r    {consis}  & 0.5886 & 0.1735 & 0.2763  & 0.6598 & 0.1029 & 0.1803  & 0.7268 & 0.0288 & 0.0528 \\
    {logit}   & 0.6374 & 0.1537 & 0.2442  & 0.7486 & 0.0939 & 0.1652  & 0.8886 & 0.0407 & 0.0471
    \end{tabular}\\
    
    
    % ~\\
    \begin{tabular}{
        S
        % P{min=0.6523, max=0.7296, first color=green, second color=orange}{}
        P{min=0.5748, max=0.6675, first color=green, second color=orange}{}
        P{min=0.0541, max=0.1698, first color=orange, second color=green}{}
        P{min=0.2134, max=0.237, first color=orange, second color=green}{}
        % P{min=0.8245, max=0.8381, first color=green, second color=orange}{}
        P{min=0.6273, max=0.858, first color=green, second color=orange}{}
        P{min=0.0668, max=0.0849, first color=orange, second color=green}{}
        P{min=0.1182, max=0.1507, first color=orange, second color=green}{}
        % P{min=0.9512, max=0.9719, first color=green, second color=orange}{}
        P{min=0.7038, max=0.9586, first color=green, second color=orange}{}
        P{min=0.035, max=0.1439, first color=orange, second color=green}{}
        P{min=0.0211, max=0.0881, first color=orange, second color=green}{}}
    \multicolumn{10}{c}{GPT-3.5-Turbo}            \\
    % \multicolumn{1}{c}{conf}          & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}         & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}         & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     \\
    {verbal}  & 0.5804 & 0.0541 & 0.2134  & 0.6273 & 0.0849 & 0.1507  & 0.7884 & 0.1439 & 0.0881 \\
    {consis}  & 0.5748 & 0.1698 & 0.237   & 0.6715 & 0.0699 & 0.1276  & 0.7038 & 0.035  & 0.022  \\
    {logit}   & 0.6675 & 0.1505 & 0.2189  & 0.858  & 0.0668 & 0.1182  & 0.9586 & 0.0449 & 0.0211
    \end{tabular} \\
    % ~\\

    \begin{tabular}{
        S
        % P{min=0.5796, max=0.7099, first color=green, second color=orange}{}
        P{min=0.5002, max=0.645, first color=green, second color=orange}{}
        P{min=0.0477, max=0.2125, first color=orange, second color=green}{}
        P{min=0.2218, max=0.3157, first color=orange, second color=green}{}
        % P{min=0.6682, max=0.7808, first color=green, second color=orange}{}
        P{min=0.5013, max=0.762, first color=green, second color=orange}{}
        P{min=0.0663, max=0.1616, first color=orange, second color=green}{}
        P{min=0.1732, max=0.2494, first color=orange, second color=green}{}
        % P{min=0.6324, max=0.9242, first color=green, second color=orange}{}
        P{min=0.4952, max=0.9093, first color=green, second color=orange}{}
        P{min=0.093, max=0.2195, first color=orange, second color=green}{}
        P{min=0.0688, max=0.2538, first color=orange, second color=green}{}}
    \multicolumn{10}{c}{Mixtral-8x7b}            \\
    % \multicolumn{1}{c}{conf}            & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}       & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}       & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}\\
    {verbal}  & 0.5002 & 0.0804 & 0.2601  & 0.5013 & 0.1616 & 0.2494  & 0.4952 & 0.1618 & 0.2538 \\
    {consis}  & 0.5318 & 0.2125 & 0.3157  & 0.7162 & 0.1121 & 0.2142  & 0.7324 & 0.093  & 0.0688 \\
    {logit}  & 0.645  & 0.0477 & 0.2218  & 0.762  & 0.0663 & 0.1732  & 0.9093 & 0.2195 & 0.106 
    \end{tabular}
    \end{tabular}
    % }
    }
\caption{Calibration performance of three mainstream confidence estimation methods}
\label{table: conf 3 method}
\end{table*}







==> _tables/gpt35-conf.tex <==
\begin{table*}[]
\scalebox{0.6}{
\begin{tabular}{
    S
    P{min=0.6523, max=0.7296, first color=green, second color=orange}{}
    P{min=0.5748, max=0.6675, first color=green, second color=orange}{}
    P{min=0.0541, max=0.1698, first color=orange, second color=green}{}
    P{min=0.2134, max=0.237, first color=orange, second color=green}{}
    P{min=0.8245, max=0.8381, first color=green, second color=orange}{}
    P{min=0.6273, max=0.858, first color=green, second color=orange}{}
    P{min=0.0668, max=0.0849, first color=orange, second color=green}{}
    P{min=0.1182, max=0.1507, first color=orange, second color=green}{}
    P{min=0.9512, max=0.9719, first color=green, second color=orange}{}
    P{min=0.7038, max=0.9586, first color=green, second color=orange}{}
    P{min=0.035, max=0.1439, first color=orange, second color=green}{}
    P{min=0.0211, max=0.0881, first color=orange, second color=green}{}}
\multicolumn{1}{c}{conf}       & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     \\
{verbal} & 0.6523 & 0.5804 & 0.0541 & 0.2134 & 0.8245 & 0.6273 & 0.0849 & 0.1507 & 0.9512 & 0.7884 & 0.1439 & 0.0881 \\
{consis} & 0.7296 & 0.5748 & 0.1698 & 0.237  & 0.8373 & 0.6715 & 0.0699 & 0.1276 & 0.9719 & 0.7038 & 0.035  & 0.022  \\
{logit}  & 0.7233 & 0.6675 & 0.1505 & 0.2189 & 0.8381 & 0.858  & 0.0668 & 0.1182 & 0.9719 & 0.9586 & 0.0449 & 0.0211
\end{tabular}}
\caption{gpt35-conf}
\label{table: gpt35 conf}
\end{table*}

==> _tables/gpt35-prompt-format.tex <==
\begin{table*}[]
\scalebox{0.6}{
\begin{tabular}
% {ccccccccccccc}
{
    S
    P{min=0.6869, max=0.7291, first color=green, second color=orange}{}
    P{min=0.6375, max=0.6832, first color=green, second color=orange}{}
    P{min=0.1505, max=0.1905, first color=orange, second color=green}{}
    P{min=0.2189, max=0.2483, first color=orange, second color=green}{}
    P{min=0.8274, max=0.8521, first color=green, second color=orange}{}
    P{min=0.8004, max=0.858, first color=green, second color=orange}{}
    P{min=0.0668, max=0.0901, first color=orange, second color=green}{}
    P{min=0.1182, max=0.1405, first color=orange, second color=green}{}
    P{min=0.9593, max=0.9843, first color=green, second color=orange}{}
    P{min=0.9106, max=0.9732, first color=green, second color=orange}{}
    P{min=0.0289, max=0.0475, first color=orange, second color=green}{}
    P{min=0.0153, max=0.0303, first color=orange, second color=green}{}
  }
\multicolumn{1}{c}{Prompt}   & \multicolumn{4}{c}{implicit}      & \multicolumn{4}{c}{sbic}          & \multicolumn{4}{c}{toxigen}       \\
\multicolumn{1}{c}{-}  & \multicolumn{1}{c}{F1}      & \multicolumn{1}{c}{AUC}    & \multicolumn{1}{c}{ECE} & \multicolumn{1}{c}{BS}    & \multicolumn{1}{c}{F1}   & \multicolumn{1}{c}{AUC}  & \multicolumn{1}{c}{ECE}  & \multicolumn{1}{c}{BS} & \multicolumn{1}{c}{F1}    & \multicolumn{1}{c}{AUC}    & \multicolumn{1}{c}{ECE} & \multicolumn{1}{c}{BS}     \\
{choice}   & 0.7286   & 0.6458 & 0.1874 & 0.2483 & 0.8508 & 0.8109 & 0.0755 & 0.1254 & 0.9843  & 0.9732 & 0.0467 & 0.0153 \\
{explain}  & 0.7291   & 0.6537 & 0.1708 & 0.2295 & 0.8377 & 0.8182 & 0.0827 & 0.1322 & 0.9719  & 0.9106 & 0.0312 & 0.0262 \\
{mask}     & 0.715    & 0.6832 & 0.1772 & 0.2324 & 0.8521 & 0.8234 & 0.0694 & 0.1225 & 0.9597  & 0.9632 & 0.0475 & 0.0238 \\
{qa}       & 0.687    & 0.6376 & 0.1905 & 0.2462 & 0.8314 & 0.834  & 0.0901 & 0.1377 & 0.9721  & 0.9238 & 0.0289 & 0.0261 \\
{target}   & 0.6981   & 0.6576 & 0.1826 & 0.2406 & 0.8274 & 0.8004 & 0.0895 & 0.1405 & 0.9593  & 0.9357 & 0.0297 & 0.0303 \\
{ensemble} & 0.7233   & 0.6675 & 0.1505 & 0.2189 & 0.8381 & 0.858  & 0.0668 & 0.1182 & 0.9719  & 0.9586 & 0.0449 & 0.0211
\end{tabular}}
\caption{Impact of prompt style on GPT-3.5-Turbo.}
\label{table: gpt35 prompt format}
\end{table*}

==> _tables/llama2-conf.tex <==
\begin{table*}[]
\scalebox{0.6}{
\begin{tabular}
{
    S
    P{min=0.6518, max=0.686, first color=green, second color=orange}{}
    P{min=0.5648, max=0.6374, first color=green, second color=orange}{}
    P{min=0.0812, max=0.1735, first color=orange, second color=green}{}
    P{min=0.2325, max=0.2763, first color=orange, second color=green}{}
    P{min=0.7844, max=0.7949, first color=green, second color=orange}{}
    P{min=0.5861, max=0.7486, first color=green, second color=orange}{}
    P{min=0.0569, max=0.1029, first color=orange, second color=green}{}
    P{min=0.1652, max=0.1811, first color=orange, second color=green}{}
    P{min=0.9176, max=0.9322, first color=green, second color=orange}{}
    P{min=0.7268, max=0.8886, first color=green, second color=orange}{}
    P{min=0.0288, max=0.1808, first color=orange, second color=green}{}
    P{min=0.0471, max=0.0891, first color=orange, second color=green}{}}
\multicolumn{1}{c}{conf}     & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}      \\
{verbal}      & 0.6518 & 0.5648 & 0.0812 & 0.2325 & 0.7844 & 0.5861 & 0.0569 & 0.1811 & 0.9176 & 0.7685 & 0.1808 & 0.0891 \\
{consis} & 0.6801 & 0.5886 & 0.1735 & 0.2763 & 0.7949 & 0.6598 & 0.1029 & 0.1803 & 0.9322 & 0.7268 & 0.0288 & 0.0528 \\
{logit}       & 0.686  & 0.6374 & 0.1537 & 0.2442 & 0.7923 & 0.7486 & 0.0939 & 0.1652 & 0.9322 & 0.8886 & 0.0407 & 0.0471
\end{tabular}}
\caption{llama2-conf-new}
\label{table: llama2 conf}
\end{table*}

==> _tables/llama2-prompt-format.tex <==
\begin{table*}[]
\scalebox{0.6}{
\begin{tabular}
% {ccccccccccccc}
{
    S
    P{min=0.6299, max=0.7248, first color=green, second color=orange}{}
    P{min=0.6141, max=0.6471, first color=green, second color=orange}{}
    P{min=0.1269, max=0.2453, first color=orange, second color=green}{}
    P{min=0.2416, max=0.2955, first color=orange, second color=green}{}
    P{min=0.7726, max=0.7957, first color=green, second color=orange}{}
    P{min=0.6928, max=0.7505, first color=green, second color=orange}{}
    P{min=0.0882, max=0.1523, first color=orange, second color=green}{}
    P{min=0.1652, max=0.2052, first color=orange, second color=green}{}
    P{min=0.8949, max=0.9333, first color=green, second color=orange}{}
    P{min=0.8227, max=0.92, first color=green, second color=orange}{}
    P{min=0.0084, max=0.0688, first color=orange, second color=green}{}
    P{min=0.0471, max=0.0776, first color=orange, second color=green}{}
  }
\multicolumn{1}{c}{Prompt}   & \multicolumn{4}{c}{implicit}      & \multicolumn{4}{c}{sbic}          & \multicolumn{4}{c}{toxigen}       \\
\multicolumn{1}{c}{-}  & \multicolumn{1}{c}{F1}      & \multicolumn{1}{c}{AUC}    & \multicolumn{1}{c}{ECE} & \multicolumn{1}{c}{BS}    & \multicolumn{1}{c}{F1}   & \multicolumn{1}{c}{AUC}  & \multicolumn{1}{c}{ECE}  & \multicolumn{1}{c}{BS} & \multicolumn{1}{c}{F1}    & \multicolumn{1}{c}{AUC}    & \multicolumn{1}{c}{ECE} & \multicolumn{1}{c}{BS}     \\
{choice}   & 0.6505 & 0.6278 & 0.1269 & 0.2416 & 0.7934 & 0.7505 & 0.0882 & 0.1667 & 0.9136 & 0.924  & 0.0688 & 0.0517 \\
{explain}  & 0.6299 & 0.6313 & 0.2145 & 0.2794 & 0.7726 & 0.7358 & 0.1391 & 0.1907 & 0.9084 & 0.9017 & 0.0367 & 0.0564 \\
{mask}     & 0.7248 & 0.6471 & 0.2453 & 0.2955 & 0.7957 & 0.6957 & 0.1523 & 0.2052 & 0.8949 & 0.8767 & 0.0133 & 0.0776 \\
{qa}       & 0.6425 & 0.637  & 0.2363 & 0.2873 & 0.7863 & 0.6928 & 0.1289 & 0.1855 & 0.9243 & 0.8227 & 0.0084 & 0.0585 \\
{target}   & 0.7005 & 0.6141 & 0.2348 & 0.2943 & 0.7893 & 0.7203 & 0.141  & 0.1961 & 0.9333 & 0.8799 & 0.0255 & 0.048  \\
{ensemble} & 0.686  & 0.6374 & 0.1537 & 0.2442 & 0.7923 & 0.7486 & 0.0939 & 0.1652 & 0.9322 & 0.8886 & 0.0407 & 0.0471
\end{tabular}}
\caption{Impact of prompt style on llama2-7b.}
\label{table: llama prompt format}
\end{table*}

==> _tables/mixtral-conf.tex <==

\begin{table*}[]
\scalebox{0.6}{
\begin{tabular}{
    S
    P{min=0.5796, max=0.7099, first color=green, second color=orange}{}
    P{min=0.5002, max=0.645, first color=green, second color=orange}{}
    P{min=0.0477, max=0.2125, first color=orange, second color=green}{}
    P{min=0.2218, max=0.3157, first color=orange, second color=green}{}
    P{min=0.6682, max=0.7808, first color=green, second color=orange}{}
    P{min=0.5013, max=0.762, first color=green, second color=orange}{}
    P{min=0.0663, max=0.1616, first color=orange, second color=green}{}
    P{min=0.1732, max=0.2494, first color=orange, second color=green}{}
    P{min=0.6324, max=0.9242, first color=green, second color=orange}{}
    P{min=0.4952, max=0.9093, first color=green, second color=orange}{}
    P{min=0.093, max=0.2195, first color=orange, second color=green}{}
    P{min=0.0688, max=0.2538, first color=orange, second color=green}{}}
\multicolumn{1}{c}{conf}         &  \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}\\
{verbal}      & 0.5796 & 0.5002 & 0.0804 & 0.2601 & 0.6682 & 0.5013 & 0.1616 & 0.2494 & 0.6324 & 0.4952 & 0.1618 & 0.2538 \\
{consis} & 0.7032 & 0.5318 & 0.2125 & 0.3157 & 0.7466 & 0.7162 & 0.1121 & 0.2142 & 0.9202 & 0.7324 & 0.093  & 0.0688 \\
{logit}       & 0.7099 & 0.645  & 0.0477 & 0.2218 & 0.7808 & 0.762  & 0.0663 & 0.1732 & 0.9242 & 0.9093 & 0.2195 & 0.106 
\end{tabular}}
\caption{mixtral-conf}
\label{table: mixtral conf}
\end{table*}


==> _tables/mixtral-prompt-format.tex <==
\begin{table*}[]
\scalebox{0.6}{
\begin{tabular}
% {ccccccccccccc}
{
    S
    P{min=0.6689, max=0.7099, first color=green, second color=orange}{}
    P{min=0.6271, max=0.7542, first color=green, second color=orange}{}
    P{min=0.0257, max=0.2419, first color=orange, second color=green}{}
    P{min=0.2093, max=0.2768, first color=orange, second color=green}{}
    P{min=0.6667, max=0.8248, first color=green, second color=orange}{}
    P{min=0.7282, max=0.8363, first color=green, second color=orange}{}
    P{min=0.0663, max=0.1839, first color=orange, second color=green}{}
    P{min=0.1364, max=0.2459, first color=orange, second color=green}{}
    P{min=0.28, max=0.9266, first color=green, second color=orange}{}
    P{min=0.8418, max=0.9369, first color=green, second color=orange}{}
    P{min=0.1016, max=0.2726, first color=orange, second color=green}{}
    P{min=0.0652, max=0.2106, first color=orange, second color=green}{}
  }
\multicolumn{1}{c}{Prompt}   & \multicolumn{4}{c}{implicit}      & \multicolumn{4}{c}{sbic}          & \multicolumn{4}{c}{toxigen}       \\
\multicolumn{1}{c}{-}  & \multicolumn{1}{c}{F1}      & \multicolumn{1}{c}{AUC}    & \multicolumn{1}{c}{ECE} & \multicolumn{1}{c}{BS}    & \multicolumn{1}{c}{F1}   & \multicolumn{1}{c}{AUC}  & \multicolumn{1}{c}{ECE}  & \multicolumn{1}{c}{BS} & \multicolumn{1}{c}{F1}    & \multicolumn{1}{c}{AUC}    & \multicolumn{1}{c}{ECE} & \multicolumn{1}{c}{BS}     \\
{choice}   & 0.6796 & 0.7099 & 0.0948 & 0.2361 & 0.6667 & 0.8363 & 0.1839 & 0.2459 & 0.28   & 0.8418 & 0.2726 & 0.2106 \\
{explain}  & 0.7004 & 0.6683 & 0.0393 & 0.2093 & 0.8248 & 0.7872 & 0.0913 & 0.1364 & 0.9266 & 0.9369 & 0.1274 & 0.0652 \\
{mask}     & 0.6689 & 0.7542 & 0.2419 & 0.2768 & 0.7165 & 0.7695 & 0.157  & 0.2166 & 0.8794 & 0.8559 & 0.1016 & 0.0977 \\
{qa}       & 0.6822 & 0.6271 & 0.0257 & 0.2282 & 0.7333 & 0.7282 & 0.0938 & 0.2041 & 0.9105 & 0.8819 & 0.2651 & 0.138  \\
{target}   & 0.6934 & 0.6785 & 0.0278 & 0.2102 & 0.8163 & 0.7814 & 0.1003 & 0.1416 & 0.8881 & 0.8883 & 0.1539 & 0.1043 \\
{ensemble} & 0.7099 & 0.645  & 0.0477 & 0.2218 & 0.7808 & 0.762  & 0.0663 & 0.1732 & 0.9242 & 0.9093 & 0.2195 & 0.106 
\end{tabular}}
\caption{Impact of prompt style on Mixtral-8x7b.}
\label{table: mixtral prompt format}
\end{table*}


==> _tables/motivation.tex <==
\begin{table}[t]
\caption{Comparison with existing FL frameworks.}
\label{table:FL framework comparison}
% \vskip -0.1in
\vspace{-3mm}
\begin{center}
\begin{normalsize}
% \begin{sc}
\scalebox{0.8}{
% \begin{tabular}{lcccr}
\begin{tabular}{llccccc}
\toprule
Features                  & implicit expressions      & prompt format       & temperature sampling & skewness & uncertainty calibration & multiple models \\
\midrule
implicit expressions               & $\dagger$ & $\dagger$ & $\surd$   & $\surd$   & $\surd$   & $\surd$ \\
prompt format          & $\times$  & $\times$  & $\dagger$ & $\dagger$ & $\dagger$ & $\surd$ \\
temperature,sampling      & $\times$  & $\times$  & $\times$ & $\dagger$ & $\dagger$ & $\surd$ \\
skewness & $\times$  & $\times$  & $\times$  & $\dagger$  & $\dagger$  & $\surd$ \\
uncertainty calibration               & $\times$  & $\dagger$   & $\dagger$   & $\dagger$   & $\dagger$   & $\surd$ \\
multiple models             & $\times$  & $\dagger$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ \\

\bottomrule
\end{tabular}}
% \end{sc}
$\times$ means no support; $\surd$ means fully support; 

$\dagger$ means partially support.
\end{normalsize}
\end{center}
% \vskip -0.5in
\vspace{-10mm}
\end{table}





% \begin{table}[t]
% \caption{Comparison with existing FL frameworks.}
% \label{table:FL framework comparison}
% % \vskip -0.1in
% \vspace{-3mm}
% \begin{center}
% \begin{normalsize}
% % \begin{sc}
% \scalebox{0.8}{
% % \begin{tabular}{lcccr}
% \begin{tabular}{llccccc}
% \toprule
% Features                  & \cite{li2023hot}      & \cite{khatun2023reliability}       & \cite{yang2023hare} & \cite{huang2023chatgpt} & FedScale & Ours \\
% \midrule
% implicit expressions               & $\dagger$ & $\dagger$ & $\surd$   & $\surd$   & $\surd$   & $\surd$ \\
% prompt format          & $\times$  & $\times$  & $\dagger$ & $\dagger$ & $\dagger$ & $\surd$ \\
% temperature,sampling      & $\times$  & $\times$  & $\times$ & $\dagger$ & $\dagger$ & $\surd$ \\
% skewness & $\times$  & $\times$  & $\times$  & $\dagger$  & $\dagger$  & $\surd$ \\
% uncertainty calibration               & $\times$  & $\dagger$   & $\dagger$   & $\dagger$   & $\dagger$   & $\surd$ \\
% multiple models             & $\times$  & $\dagger$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ \\

% \bottomrule
% \end{tabular}}
% % \end{sc}
% $\times$ means no support; $\surd$ means fully support; 

% $\dagger$ means partially support.
% \end{normalsize}
% \end{center}
% % \vskip -0.5in
% \vspace{-10mm}
% \end{table}



==> _txt/backup.tex <==

Table~\ref{tab:conf compare} shows the confidence calibration comparison on GPT-3.5-Turbo. 


\textbf{Takeaway \ding{172}:}, From the aspect of uncertainty strategy: MoP performs better than other uncertainty strategies. 

\textbf{Takeaway \ding{173}:}, From the aspect of confidence policy: mean-sd usually performs better than others, then mean. while mutual performs better in CoT SC setting. 

\textbf{Takeaway \ding{174}:}, Consistency as confidence policy performs the worst, with a big gap from the others.



\begin{table*}
\centering
% \begin{tabular}{clllllll}
\begin{tabular}{
    S
    S
    P{min=0.5851, max=0.6669, first color=green, second color=orange}{}
    P{min=0.1417, max=0.1889, first color=orange, second color=green}{}
    P{min=0.6432, max=0.8580, first color=green, second color=orange}{}
    P{min=0.0484, max=0.0884, first color=orange, second color=green}{}
    P{min=0.7038, max=0.9607, first color=green, second color=orange}{}
    P{min=0.0298, max=0.1932, first color=orange, second color=green}{}
  }
\hline
\multicolumn{2}{c}{Method}   & \multicolumn{2}{c}{Implicit}                            & \multicolumn{2}{c}{SBIC}                                & \multicolumn{2}{c}{ToxiGen}                       \\ \hline
{strategy}      & {conf policy} & \multicolumn{1}{c}{AUC}       & \multicolumn{1}{c}{ECE} & \multicolumn{1}{c}{AUC}       & \multicolumn{1}{c}{ECE} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{ECE} \\ \hline
{Verbal}        &   {-}           & 0.6240                        & 0.1889                  & 0.8264                        & 0.0884                  & 0.9197                  & 0.0298                  \\ \hline
{CoT SC}        & {consistency}  & 0.5851                        & 0.1840                  & 0.6432                        & 0.0674                  & 0.7911                  & 0.0481                  \\
              & {mean}         & 0.6054                        & 0.1610                  & 0.6928                        & 0.0608                  & 0.7251                  & 0.1190                  \\
              & {mean-sd}      & 0.6097                        & 0.1706                  & 0.6981                        & 0.0642                  & 0.7681                  & 0.1932                  \\
              & {mutual}       & 0.6476                        & 0.1802                  & 0.7622                        & 0.0643                  & 0.7970                  & 0.0616                  \\ \hline
{Demonstration} & {consistency}  & 0.5852               & 0.1734                           &  0.6089                       & 0.0813                  & 0.7327                  & 0.0474                  \\
              & {mean}         & 0.6541                        & 0.1545                  & 0.8165                        & 0.0737                  & 0.9106                  & 0.0401                  \\
              & {mean-sd}      & 0.6547                        & 0.1419                  & 0.8130                        & 0.0746                  & 0.9112                  & 0.0448                  \\
              & {mutual}       & 0.6518                        & 0.1735                  & 0.8096                        & 0.0781                  & 0.9163                  & 0.0327                  \\ \hline
{Prompt Style}  & {consistency}  & 0.5884                        & 0.1679                  & 0.6689                        & 0.0706                  & 0.7038                  & 0.0349                  \\
              & {mean}         & 0.6674                        & 0.1505                  & 0.8580                        & 0.0667                  & 0.9586                  & 0.0448                  \\
              & {mean-sd}      & 0.6669                        & 0.1417                  & 0.8561                        & 0.0484                  & 0.9607                  & 0.0514                  \\
              & {mutual}       & 0.6611                        & 0.1694                  & 0.8354                        & 0.0627                  & 0.9500                  & 0.0492                  \\ \hline
\end{tabular}
\caption{Confidence Calibration Comparison on GPT-3.5-Turbo. The closer to orange the better, the closer to green the worse. Obviously, Mixture of prompt style improves LLM's calibration performance.}
\label{tab:conf compare}
\end{table*}




\begin{figure}
    \centering
    \includegraphics[width=3.33in]{_fig/experiment/prompt_diverse.pdf}
    % \vspace{-20mm}
    \caption{The performance of different prompt styles fluctuates. No specific prompt style consistently performs better.}
    \label{fig:prompt_fluctuated}
\end{figure}



Fig.~\ref{fig:prompt_fluctuated} shows the performance of individualized prompt style. We can see that the performance of different prompt styles fluctuates. No specific prompt style consistently performs better.




% % no ensemble

% \begin{table*}
% \centering
% \scalebox{0.8}{
% \begin{tabular}{
%     S
%     P{min=0.6869, max=0.7291, first color=green, second color=orange}{}
%     P{min=0.6375, max=0.6831, first color=green, second color=orange}{}
%     P{min=0.1707, max=0.1905, first color=orange, second color=green}{}
%     P{min=0.8273, max=0.8520, first color=green, second color=orange}{}
%     P{min=0.8004, max=0.8339, first color=green, second color=orange}{}
%     P{min=0.0694, max=0.0901, first color=orange, second color=green}{}
%     P{min=0.9593, max=0.9842, first color=green, second color=orange}{}
%     P{min=0.9105, max=0.9732, first color=green, second color=orange}{}
%     P{min=0.0289, max=0.0474, first color=orange, second color=green}{}
%   }
% \hline
% \multicolumn{1}{c}{Prompt} & \multicolumn{1}{c}{F1}     & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{ECE}    & \multicolumn{1}{c}{F1}     & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{ECE}    & \multicolumn{1}{c}{F1}     & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{ECE}    \\
% \hline
% {choice}                     & 0.7285 & 0.6458                  & 0.1873 & 0.8508 & 0.8108                  & 0.0754 & 0.9842 & 0.9732                  & 0.0467 \\
% {explain}                    & 0.7291 & 0.6537                  & 0.1707 & 0.8377 & 0.8182                  & 0.0826 & 0.9718 & 0.9105                  & 0.0312 \\
% {mask}                       & 0.7150 & 0.6831                  & 0.1772 & 0.8520 & 0.8233                  & 0.0694 & 0.9596 & 0.9631                  & 0.0474 \\
% {qa}                         & 0.6869 & 0.6375                  & 0.1905 & 0.8313 & 0.8339                  & 0.0901 & 0.9721 & 0.9237                  & 0.0289 \\
% {target}                     & 0.6981 & 0.6576                  & 0.1826 & 0.8273 & 0.8004                  & 0.0895 & 0.9593 & 0.9357                  & 0.0297 \\
% \hline
% \end{tabular}
% }
% \caption{Impact of prompt style on GPT-3.5-Turbo.}
% \label{tab:prompt gpt}
% \end{table*}





% \begin{table}[]
% \begin{tabular}{
%     S
%     P{min=0.6298, max=0.7247, first color=green, second color=orange}{}
%     P{min=0.6141, max=0.6470, first color=green, second color=orange}{}
%     P{min=0.1269, max=0.2453, first color=orange, second color=green}{}
%     P{min=0.77, max=0.796, first color=green, second color=orange}{}
%     P{min=0.69, max=0.75, first color=green, second color=orange}{}
%     P{min=0.09, max=0.15, first color=orange, second color=green}{}
%     P{min=0.894, max=0.914, first color=green, second color=orange}{}
%     P{min=0.822, max=0.92, first color=green, second color=orange}{}
%     P{min=0.0084, max=0.07, first color=orange, second color=green}{}
%   }
% \hline
% \multicolumn{1}{c}{Prompt}  & \multicolumn{1}{c}{F1}      & \multicolumn{1}{c}{AUC}    & \multicolumn{1}{c}{ECE}    & \multicolumn{1}{c}{F1}   & \multicolumn{1}{c}{AUC}  & \multicolumn{1}{c}{ECE}  & \multicolumn{1}{c}{F1}    & \multicolumn{1}{c}{AUC}    & \multicolumn{1}{c}{ECE}     \\
% \hline
% {choice}  & 0.6500    & 0.627  & 0.1269 & 0.790   & 0.75 & 0.09 & 0.914  & 0.920   & 0.070    \\
% {explain} & 0.6298  & 0.631  & 0.2145 & 0.770   & 0.73 & 0.14 & 0.908 & 0.901  & 0.036   \\
% {mask}    & 0.7247  & 0.647  & 0.2453 & 0.796 & 0.70  & 0.15 & 0.894 & 0.876  & 0.013   \\
% {qa}      & 0.6424 & 0.637  & 0.2360  & 0.786 & 0.69 & 0.13 & 0.924 & 0.822  & 0.008 \\
% {target}  & 0.7004 & 0.614 & 0.2340  & 0.789 & 0.72 & 0.14 & 0.933 & 0.8798 & 0.025  \\
% \hline
% \end{tabular}
% \caption{Impact of prompt style on Llama-7b.}
% \label{tab:prompt llama}
% \end{table}





% \begin{table}[]
% \begin{tabular}{
% P{min=0.2158, max=0.2505, first color=orange, second color=green}{}
% P{min=0.1107, max=0.1338, first color=orange, second color=green}{}
% P{min=0.0130, max=0.0904, first color=orange, second color=green}{}
% }
% 0.2505          & 0.1253 & 0.0130 \\
% 0.2278          & 0.1195 & 0.0398 \\
% 0.2319 & 0.1216 & 0.0904 \\
% 0.2406          & 0.1209 & 0.0196 \\
% 0.2455          & 0.1415 & 0.0402 \\
% 0.2234          & 0.1307 & 0.0381 \\
% 0.2194          & 0.1295 & 0.0375 \\
% 0.2334          & 0.1338 & 0.0317 \\
% 0.2369          & 0.1275 & 0.0219 \\
% 0.2188          & 0.1182 & 0.0210 \\
% 0.2158          & 0.1107 & 0.0209 \\
% 0.2254          & 0.1192 & 0.0197
% \end{tabular}
% \caption{Brier score on GPT-3.5-Turbo.}
% \label{tab:conf compare}
% \end{table}



% \begin{table*}[]
% \scalebox{0.6}{
% \begin{tabular}{
%     S
%     S
%     P{min=0.6518, max=0.7148, first color=green, second color=orange}{}
%     P{min=0.5415, max=0.6374, first color=green, second color=orange}{}
%     P{min=0.0812, max=0.2112, first color=orange, second color=green}{}
%     P{min=0.2325, max=0.2896, first color=orange, second color=green}{}
%     P{min=0.7831, max=0.7949, first color=green, second color=orange}{}
%     P{min=0.5861, max=0.7486, first color=green, second color=orange}{}
%     P{min=0.0569, max=0.1237, first color=orange, second color=green}{}
%     P{min=0.1652, max=0.186, first color=orange, second color=green}{}
%     P{min=0.9176, max=0.9322, first color=green, second color=orange}{}
%     P{min=0.7028, max=0.8886, first color=green, second color=orange}{}
%     P{min=0.0109, max=0.1808, first color=orange, second color=green}{}
%     P{min=0.0471, max=0.0891, first color=orange, second color=green}{}}
%    \multicolumn{1}{c}{conf}         & \multicolumn{1}{c}{name}   & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     \\
% {verbal}      & {verbal} & 0.6518 & 0.5648 & 0.0812 & 0.2325 & 0.7844 & 0.5861 & 0.0569 & 0.1811 & 0.9176 & 0.7685 & 0.1808 & 0.0891 \\
% {consistency} & {demo}   & 0.7148 & 0.5415 & 0.2112 & 0.2896 & 0.7831 & 0.6243 & 0.1237 & 0.186  & 0.918  & 0.7028 & 0.0109 & 0.0587 \\
% {consistency} & {prompt} & 0.6801 & 0.5886 & 0.1735 & 0.2763 & 0.7949 & 0.6598 & 0.1029 & 0.1803 & 0.9322 & 0.7268 & 0.0288 & 0.0528 \\
% {logit}       & {demo}   & 0.7109 & 0.6139 & 0.2075 & 0.2708 & 0.7848 & 0.7409 & 0.1162 & 0.1729 & 0.918  & 0.8164 & 0.0149 & 0.0571 \\
% {logit}       & {prompt} & 0.686  & 0.6374 & 0.1537 & 0.2442 & 0.7923 & 0.7486 & 0.0939 & 0.1652 & 0.9322 & 0.8886 & 0.0407 & 0.0471
% \end{tabular}}
% \caption{llama}
% \end{table*}





% \begin{table*}[]
% \scriptsize
% \begin{tabular}{llllllllllllll}
% \multicolumn{1}{c}{conf}         & \multicolumn{1}{c}{name}   & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     \\
% verbal      & verbal & 0.5796 & 0.5002 & 0.0804 & 0.2601 & 0.6682 & 0.5013 & 0.1616 & 0.2494 & 0.6324 & 0.4952 & 0.1618 & 0.2538 \\
% consistency & demo                                  & 0.6901 & 0.6315 & 0.128  & 0.2417 & 0.8007 & 0.7324 & 0.0242 & 0.1343 & 0.9212 & 0.7235 & 0.0142 & 0.0565 \\
% consistency & prompt                                & 0.7032 & 0.5318 & 0.2125 & 0.3157 & 0.7466 & 0.7162 & 0.1121 & 0.2142 & 0.9202 & 0.7324 & 0.093  & 0.0688 \\
% logit       & demo                                  & 0.6854 & 0.6542 & 0.0732 & 0.2144 & 0.8164 & 0.7858 & 0.1979 & 0.1709 & 0.9256 & 0.8787 & 0.1647 & 0.0817 \\
% logit       & prompt                                & 0.7099 & 0.645  & 0.0477 & 0.2218 & 0.7808 & 0.762  & 0.0663 & 0.1732 & 0.9242 & 0.9093 & 0.2195 & 0.106 
% \end{tabular}
% \caption{mixtral}
% \end{table*}




% \begin{table*}[]
% \scriptsize
% \begin{tabular}{llllllllllllll}
% \multicolumn{1}{c}{conf}         & \multicolumn{1}{c}{name}   & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     & \multicolumn{1}{c}{f}      & \multicolumn{1}{c}{auc}    & \multicolumn{1}{c}{ece}    & \multicolumn{1}{c}{bs}     \\
% verbal & verbal & 0.6523 & 0.5804 & 0.0541 & 0.2134 & 0.8245 & 0.6273 & 0.0849 & 0.1507 & 0.9512 & 0.7884 & 0.1439 & 0.0881 \\
% consis & demon                                 & 0.6876 & 0.5925 & 0.1702 & 0.2456 & 0.829  & 0.6089 & 0.0796 & 0.1416 & 0.9426 & 0.7752 & 0.0401 & 0.0403 \\
% consis & prompt                                & 0.7296 & 0.5748 & 0.1698 & 0.237  & 0.8373 & 0.6715 & 0.0699 & 0.1276 & 0.9719 & 0.7038 & 0.035  & 0.022  \\
% logit  & demo                                  & 0.6908 & 0.6541 & 0.1546 & 0.2234 & 0.8281 & 0.8165 & 0.0738 & 0.1307 & 0.9512 & 0.9106 & 0.0401 & 0.0382 \\
% logit  & prompt                                & 0.7233 & 0.6675 & 0.1505 & 0.2189 & 0.8381 & 0.858  & 0.0668 & 0.1182 & 0.9719 & 0.9586 & 0.0449 & 0.0211
% \end{tabular}
% \caption{gpt35}
% \end{table*}


==> _txt/v01_5_result_calibration.tex <==


\section{Results of Confidence Calibration}

\input{_tables/conf_combine}
\input{_fig/conf_scenario}

% 另一种写法。
% logit-based method的auc在所有模型所有数据集都表现最好。这是因为，和verbal-based method相比，xxx;和consistency-based method相比，xxx.
% ece指标要结合task itself accuracy和logit分布，分类讨论。

Table ~\ref{table: conf 3 method} shows the comparison of three main stream confidence estimation methods. 
% 我们发现不同的不确定性估计方法在校准上的表现受到任务本身的表现以及模型本身的概率分布的影响。我们根据任务本身的表现和模型本身的概率分布分类成几个场景，并讨论了不同方法的优势和劣势。
We found that the calibration performance of various uncertainty estimation methods is influenced by both the performance of the task itself and the probability distribution of the model. We categorized them into several scenarios based on the task performance and the model's probability distribution, and discussed the advantages and disadvantages of different uncertainty estimation methods.


% (1) 在任务本身准确率不高且confidence体现出overconfident的情况下(模型llama在数据集implicit和sbic, 模型gpt35在数据集implicit)，verbal-based method取得了几乎最好的ece值和bs值，而auc值却几乎最差。比如说在implicit数据集上,verbal-based method的ece是最好的0.0812，远远好于logit-based method的ece（0.1537）.而auc的趋势确实相反的，verbal-based method的auc是0.5648,远低于logit-based方法的0.6374。
\subsection{When can verbal-based method be better?}

\textbf{(Scenario 1) In cases where the accuracy of the task itself is not high and the model's token logit reflects an overconfident situation (model llama on the implicit and sbic datasets, model gpt35 on the implicit dataset), the verbal-based method achieved nearly the best ECE and BS, while the AUC were almost the worst.} For example, on the implicit dataset, the ECE of the verbal-based method was the best at 0.0812, significantly outperforming the logit-based method with an ECE of 0.1537. However, the trend for AUC was the opposite, with the verbal-based method having an AUC of 0.5648, much lower than the logit-based method's 0.6374.

\input{_fig/conf_compare_verbal_logit}

% verbal-based method的ece比logit-based方法的ece好。logit-based method和consistency-based method都overconfident，confidence分布集中于大于0.9的区间，但是这个区间的准确率却不那么高，因此导致confidence低于预期准确率，出现了under-calibrated的校准误差（图2b）. 而verbal-based的方法对confidence估计比较保守，confidence分布大多集中在0.7-0.8，与准确率相近，所以校准误差较小(图2a)。


% 然而，logits方法的AUC要高于verbal-based方法。我们发现，在同一confidence阈值下，verbal-based方法和logit-based方法的fpr相近，而logit-based方法的confidence distribution更加overconfident，导致true postive越大，所以tpr越大，ROC曲线越高（如图2c所示）。以阈值0.7为例，fpr都是59，而verbal的tpr是67，logit-based的tpr是78，所以logit的曲线要高于verbal，具体分析详见appendix。

\textbf{Why does verbal-based method achieve best ece in such senario?} 
% This is because both the logit-based method and the consistency-based method tend to be overconfident, deviating significantly from the high accuracy associated with the confidence interval in ideal calibration. In contrast, the verbal-based method does not exhibit overconfidence and is closer to the accuracy that is not particularly emphasized by the task itself.
The ECE of the verbal-based method is better than that of the logit-based method. Both the logit-based method and the consistency-based method exhibit overconfidence, with confidence distributions concentrated in the interval greater than 0.9. However, the accuracy within this interval is not very high, leading to confidence levels lower than the expected accuracy and resulting in under-calibrated calibration errors (Fig.~\ref{fig: conf-compare-verbal-logit} b). In contrast, the verbal-based method provides a more conservative estimate of confidence, with the distribution mostly concentrated in the range of 0.7-0.8, close to the accuracy, resulting in smaller calibration errors (Fig.~\ref{fig: conf-compare-verbal-logit} a).

\textbf{Why does verbal-based method achieve worst auc in such senario?} The AUC of the logit-based method is higher than that of the verbal-based method. We observed that, at the same confidence threshold, the fpr of the verbal-based method and the logit-based method are similar. However, the confidence distribution of the logit-based method is more overconfident, leading to a larger true positive, resulting in a higher tpr and a higher ROC curve (as shown in Fig.~\ref{fig: conf-compare-verbal-logit} c). For example, at a threshold of 0.7, both methods have an fpr of 59, but the verbal-based tpr is 67, and the logit-based tpr is 78, causing the logit curve to be higher than the verbal curve. Detailed analysis is provided in the appendix.



% (2) 在任务本身准确率高且confidence普遍比较高的情况下 (模型llama在数据集toxigen, 模型gpt35在数据集sbic和toxigen)，verbal-based method在ece上也失去了优势。这是因为toxigen上已经over-calibrated。即使是在简单的数据集上，verbal conf依然主要预测成0.7-0.8，而简单数据集上准确率很高，但confidence却没有对应地升高，导致over-calibrate,acc高于conf的误差很大。说明verbal其实不能良好地随着对不同数据表达出差异化的confidence。verbal confidence是受了demonstration的影响。
\input{_fig/conf_over_calibrate}

\subsection{When can logit-based method be better?}

\textbf{logit-based method achieve best AUC in all senarios (ranging from all models and all datasets).} Comparison and analysis with verbal-based method can be found in the last section, comparison with consistency-based method can be found in the next section. Next, we discuss the advantages of logit-based method in ECE.
% 要不要把上一个section里的auc那段挪下来放在这分析为什么logit的auc好，这样的话consistency感觉也得挪下来。


\textbf{(Scenario 2) In cases where the task itself has high accuracy and confidence is generally high (model llama on the toxigen dataset, model gpt35 on the sbic and toxigen datasets), logit-based method achieves best ECE while the verbal-based method loses its advantage in ECE.} This is because on simple datasets, the task accuracy is very high, so the logit-based method with high confidence tends to be closer to the high accuracy, while the verbal-based method maintains a conservative confidence, significantly lower than the accuracy. As shown in Fig.~\ref{fig: conf-over-calibrate}, even on a simple dataset, verbal confidence predominantly predicts values in the range of 0.7-0.8. Despite the high accuracy on the simple dataset, the confidence does not correspondingly increase, leading to over-calibration. The error is substantial when accuracy is much higher than confidence. This indicates that verbal cannot effectively differentiate confidence across different datasets, as verbal confidence is influenced by demonstrations.



% (3) 在模型本身的logit分布不普遍过高时(模型mixtral-8x7b)，logit已经很好地校准了，所以verbal没有展示出优势。如图6所示，不同于其他模型分布在分数较高的区间，mixtral模型的logit主要分布在0.5-0.6区间内,比较接近于准确率，具有较好的校准能力。所以在logit方法在auc,ece,bs上都取得了最好的值。

\textbf{(Scenario 3) In cases where the model's token logit distribution is not generally too high (model mixtral-8x7b), the logit is already well-calibrated, and verbal does not demonstrate superiority.} As shown in Fig.~\ref{fig: temperature-bar} a, unlike other models that have distributions in higher score ranges, the logit of the mixtral model is mainly distributed in the 0.5-0.6 range, closely resembling the accuracy and exhibiting good calibration ability. Therefore, the logit method achieves the best values in terms of AUC, ECE, and BS.

% (4) consistency-based method在所有模型上表现都不好。和logit相比，因为都是overconfident，所以在ece上差距不大,但auc低于logit-based method. 这是因为consistency score受multi-inference次数的影响，主要集中的几个离散值上（3/5，4/5，5/5），导致计算auc时confidence threshold取的比较少（图4a）。而logit方法的confidence score能取到很多连续值(图4b)。confidence的分布影响了auc的计算。例如在图4c中，当threshold取0.8时，两种方法的roc曲线上的点很接近，然而当logit conf在threshold取0.99至0.8时，fpr从0.01到0.64都有，而consistency方法这部分是缺失的。这说明consistenty-based method的confidence值的离散性导致了uncertainty的表达能力受限。

\subsection{When can consistency-based method be better?}

\textbf{The consistency-based method performs poorly across all models. Compared to logit-based method, the difference in ECE is not significant since both methods are overconfident. However, the AUC is lower for the consistency-based method compared to the logit-based method.} This is because the consistency score is influenced by the number of multi-inferences, mainly concentrated on a few discrete values (3/5, 4/5, 5/5), leading to fewer confidence thresholds considered when calculating AUC (Fig.~\ref{fig: conf-compare-consistency-logit} a). In contrast, the logit method's confidence score covers many continuous values (Fig.~\ref{fig: conf-compare-consistency-logit} b), influencing the calculation of AUC. For example, in Fig.~\ref{fig: conf-compare-consistency-logit} c, when the threshold is set at 0.8, the points on the ROC curves for both methods are close. However, for logit confidence, ranging from 0.99 to 0.8, there are corresponding fpr values from 0.01 to 0.64, while for the consistency-based method, this portion is missing. This indicates that the discreteness of confidence values in the consistency-based method limits its ability to express uncertainty.


\input{_fig/conf_compare_consistency_logit}


% 应该加一组实验，探究demonstration对verbal的影响。分别是zero-shot, 70(完成), 95




\subsection{The common drawbacks of the three methods}
An ideal confidence estimation method should have high confidence for correctly predicted data and low confidence for incorrectly predicted data. However, 
Fig.~\ref{fig: confidence discriminability} shows that confidence distributions of correctly classified and misclassified cases overlap significantly, indicating these existing methods struggle to distinguish the confidence between incorrectly predicted and correctly predicted instances.






\subsection{Effect of In-context Learning Factors}

We investigate the impact of various in-context learning factors, including prompt format, parameters of temperature and top p, and demonstrations.

% 不同的prompt在calibration和task performance的表现是波动的，没有哪种prompt更好。在不同的模型不同数据集上，任何一种prompt都能达到最好或最差的表现。但我们发现prompt ensemble后的结果在任务表现和不确定度校准表现上都取得了一个较好的效果，不会出现较差的结果。这可能是因为不同prompt使模型产生更多样化的结果，在多样化的结果下仍然能保持一致的答案说明模型比较确定且效果较好。


\textbf{Effects of prompt format on calibration.}
Table ~\ref{table: llama prompt format}, Table ~\ref{table: mixtral prompt format}, Table ~\ref{table: gpt35 prompt format} show that the performance of different prompts varies in both calibration and task performance; There is no prompt that is consistently better. Across different models and datasets, any given prompt can achieve either the best or worst performance. 
% gpt35在implicit数据集上auc最好的是mask，在sbic数据集上auc最好的是qa,ece最好的是mask, toxigen上最好的是choice,ece最好的是qa和target

% llama2在implicit数据集上auc最好的是mask,ece,bs最好的是choice，sbic上auc,ece,bs最好的都是choice,toxigen上auc最好的是choice，ece最好的是qa,bs最好的是target.


However, we observe that the ensemble of responses from different prompts shows a better overall effect in both task performance and uncertainty calibration. This might be attributed to the diverse outcomes generated by different prompts. Even with diverse results, the consistent answers indicate that the model is more certain and performs better in such diverse scenarios.

% \textbf{Effects of demonstration.} 
\textbf{Effects of demonstration.}
We also explore the potential of ensemble method changing demonstrations. We fix the prompt format as vanilla QA and randomly change balanced demonstrations in each round of single inference. With an increase in the number of rounds, there is a slight improvement in the model's results, but it is not as effective as the ensemble method based on prompts. 

\textbf{Effects of parameters of temperature and sampling.}
Fig.~\ref{fig: temperature} shows the calibration performance when changing temperature scaling and decoding sampling. \textbf{We find that due to differences in the logit distribution, models exhibit varying sensitivities to temperature and sampling parameters, sometimes even in opposite tends.}
We fix the top p as 1 and change the temperature. 
As the temperature increases, Llama achieves better calibration performance (both AUC and ECE). However, Mixtral remained relatively stable in AUC, and its performance improved and then deteriorated in terms of ECE.
We fix the temperature as 1 and change the sampling parameter top p. We find that 
As the top-p value increased, Llama demonstrated improved calibration performance, while Mixtral showed a deterioration in calibration performance according to the ECE metric.
These phenomena arise because of the different logit distribution as shown in Fig. ~\ref{fig: temperature-bar}. 
The logit distribution of Mixtral is primarily concentrated between 0.5 and 0.7, while Llama's logit is mainly distributed between 0.9 and 1.0. This indicates that Llama is over confident, whereas Mixtral exhibits a more cautious level of confidence. As the temperature increases, the logit distribution of Mixtral becomes sharper, leading to over-calibration. On the other hand, the logit distribution of Llama becomes smoother, enhancing its ability to differentiate confidence levels.







\begin{figure}
    \centering
    \includegraphics{_fig/experiment/temperature.pdf}
    % \vspace{-20mm}
    \caption{The impact of temperature and top p we fix t=1, change top p. we fix top p=1, change temperature. (1) The performance change greatly, which means t and p are important for calibration. (2) Llama2 and Mixtral show different tends, suggesting the adjustment of t,p should be customized on different models.}
    \label{fig: temperature}
\end{figure}


\begin{figure}
    \centering
    \includegraphics{_fig/experiment/temperature-bar.pdf}
    % \vspace{-20mm}
    \caption{The logit distribution and confidence bin of Llama and Mixtral.}
    \label{fig: temperature-bar}
\end{figure}


\begin{figure}
    \centering
    \includegraphics{_fig/experiment/distribution_implicit.pdf}
    \vspace{-20mm}
    \caption{The confidence distributions of correctly classified and misclassified cases overlap significantly, indicating that the existing uncertainty estimation methods can not effectively differentiate confidence in predictions.}
    \label{fig: confidence discriminability}
\end{figure}



% \input{_tables/llama2-conf}

% \input{_tables/mixtral-conf}

% \input{_tables/gpt35-conf}


\input{_tables/gpt35-prompt-format}

\input{_tables/llama2-prompt-format}

\input{_tables/mixtral-prompt-format}

